Enhancing Structured-Data Retrieval with GraphRAG: Soccer Data Case Study

Extracting meaningful insights from large and complex datasets poses significant challenges, particularly in ensuring the accuracy and relevance of retrieved information. Traditional data retrieval methods such as sequential search and index-based retrieval often fail when handling intricate and interconnected data structures, resulting in incomplete or misleading outputs. To overcome these limitations, we introduce Structured-GraphRAG, a versatile framework designed to enhance information retrieval across structured datasets in natural language queries. Structured-GraphRAG utilizes multiple knowledge graphs, which represent data in a structured format and capture complex relationships between entities, enabling a more nuanced and comprehensive retrieval of information. This graph-based approach reduces the risk of errors in language model outputs by grounding responses in a structured format, thereby enhancing the reliability of results. We demonstrate the effectiveness of Structured-GraphRAG by comparing its performance with that of a recently published method using traditional retrieval-augmented generation. Our findings show that Structured-GraphRAG significantly improves query processing efficiency and reduces response times. While our case study focuses on soccer data, the framework's design is broadly applicable, offering a powerful tool for data analysis and enhancing language model applications across various structured domains.

==> accuracy.tex <==

    
    
        
    
    
        
    
    
    
    
        
    
    
    



\begin{table}

    \centering
    \begin{tabular}{|c|c|c|c|c|c||c|c|c|c|c|}
    
        \hline
        
        \multirow{3}{1.3cm}{\textbf{Query} \\ \vspace{0.3cm} \\ \textbf{$\downarrow$ Iteration$\rightarrow$}} 
        & \multicolumn{5}{|c||}{\textbf{SoccerRAG~\cite{soccerrag}}}
        & \multicolumn{5}{|c|}{\textbf{\frameworkname}}
        \\ \hhline{~-----------}
    
        & 1 
        & 2 
        & 3 
        & 4 
        & 5 
        & 1 
        & 2 
        & 3 
        & 4 
        & 5 
        \\ \hline
        
        \multicolumn{11}{c}{} \\[-1.5ex]  %
        
        Q1 
        & \greenV 
        & \greenV 
        & \greenV 
        & \greenV 
        & \greenV 
        & \greenV
        & \greenV 
        & \greenV 
        & \greenV 
        & \greenV 
        \\ \hline
    
        Q2 
        & \redX 
        & \redX 
        & \greenV 
        & \redX 
        & \redX 
        & \greenV
        & \greenV 
        & \redX 
        & \greenV 
        & \redX 
        \\ \hline 
    
        Q3 
        & \redX 
        & \greenV 
        & \redX 
        & \redX 
        & \greenV 
        & \greenV
        & \greenV 
        & \redX 
        & \greenV 
        & \greenV 
        \\ \hline
    
        Q4 
        & \redX 
        & \redX 
        & \redX 
        & \redX 
        & \greenV 
        & \greenV
        & \redX 
        & \greenV 
        & \greenV 
        & \greenV 
        \\ \hline
    
        Q5 
        & \greenV
        & \redX 
        & \greenV 
        & \redX 
        & \greenV 
        & \greenV
        & \greenV 
        & \greenV 
        & \greenV 
        & \greenV 
        \\ \hline
        
        Q6 
        & \redX 
        & \redX 
        & \redX 
        & \redX 
        & \redX 
        & \greenV
        & \greenV 
        & \greenV 
        & \greenV 
        & \greenV 
        \\ \hline
    
    \end{tabular}
    
    \caption{Comparison of accuracy between SoccerRAG~\cite{soccerrag} and \frameworkname. Differences are highlighted with \greenV~(green check mark) and \redX~(red X).}
    \label{tab:accuracy}
    
\end{table}


==> dataset-summary-extended.tex <==
\begin{table*}

    \small
    \centering
    
    \begin{tabular}{|c|c|l|l|c|c|c|}
    
        \hline
        \textbf{Source Dataset}
        & \textbf{Component} 
        & \textbf{Corresponding File} 
        & \textbf{Type} 
        & \textbf{SoccerRAG~\cite{soccerrag,soccerrag-demo}}
        & \textbf{Soccer-GraphRAG~\cite{SepasdarIronGraph}}
        & \textbf{\frameworkname} %
        \\ \hline 

        \multirow{2}{*}{SoccerNet-Echoes~\cite{soccernet-echoes}} 
        & \multirow{2}{*}{ASR}
        & \texttt{1\_half-ASR.json} 
        & Unstructured 
        & \no
        & \yes
        & \no
        \\ \hhline{~~-----} 
        
        & 
        & \texttt{2\_half-ASR.json}
        & Unstructured 
        & \no
        & \yes
        & \no
        \\ \hline 
         
        \multirow{2}{*}{SoccerNet~\cite{SoccerNet,SoccerNetv2}} 
        & Captions 
        & \texttt{Labels-caption.json}
        & Structured 
        & \yes
        & \no
        & \yes
        \\ \hhline{~------} 
         
        & Labels
        & \texttt{Labels-v2.json}   
        & Structured 
        & \yes
        & \no
        & \yes
        \\ \hline 
    
    \end{tabular}
    \caption{Source datasets and related work.}
    \label{tab:dataset-summary}
    
\end{table*}


==> query-response-time.tex <==
\begin{table}

    \centering
    
    \begin{tabular}{|c|c|c|}
        \hline
        
        \multirow{2}{*}{\textbf{Query}} 
        & \multicolumn{2}{|c|}{\textbf{Query Response Time}} 
        \\ \hhline{~--}
        
        & \textbf{SoccerRAG~\cite{soccerrag}} 
        & \textbf{\frameworkname} 
        \\ \hline
        
        Q1 
        & 4.61 
        & 1.66 
        \\ \hline
        
        Q2 
        & 22.23 
        & 4.00 
        \\ \hline
        
        Q3 
        & 595.98 
        & 6.16 
        \\ \hline
        
        Q4 
        & 109.46 
        & 2.48 
        \\ \hline
        
        Q5 
        & 56.97 
        & 2.14 
        \\ \hline
        
        Q6 
        & 106.33 
        & 2.98 
        \\ \hline
    
    \end{tabular}
    
    \caption{Comparison of query response time between SoccerRAG~\cite{soccerrag} and \frameworkname.}
    \label{tab:query-response-time}
\end{table}

